Master's Thesis: Excitation Spectrum of a Weakly Interacting Spin-Orbit Coupled Bose-Einstein Condensate

A weakly interacting, spin-orbit coupled, two-component, ultracold Bose gas bound to a Bravais lattice is studied. Motivated by recent experimental advances in the field of synthetically spin-orbit coupled, ultracold, neutral atomic gases showing Bose-Einstein condensation, an analytic framework with which to describe such systems in the superfluid regime is presented. This is applied to a Rashba spin-orbit-coupled Bose gas in a two-dimensional optical lattice. The exotic nature of Bose-Einstein condensation in the presence of spin-orbit coupling is an interesting study by itself. Additionally, when the optical lattice is introduced, the system provides a highly controllable experimental testing ground for numerous condensed matter physics phenomena. Five phases of the system are considered, and their excitation spectra, critical superfluid velocities and free energies are found. In obtaining the free energy, the effects of terms in the Hamiltonian that are linear in excitation operators are included, and such terms have not been studied previously in this context. Minimization of the free energy at zero temperature is used to confirm the phase diagrams reported in the literature, where it has usually been obtained by neglecting the effect of excitations. The plane and stripe wave phases in the phase diagram are bosonic analogues of Fulde-Ferrell-Larkin-Ovchinnikov states in superconductors involving nonzero condensate momenta.

==> appDiagThry.tex <==
\chapter{Additional Diagonalization Theory} \label{app:Negeigenvaluediag}
% \section{Failure of Unitary Transformation}
% Assuming a matrix $T$ with the property $T^\dagger = T^{-1}$ that diagonalizes $M$ exists, we can perform the unitary trasformation $\boldsymbol{A}^{\dagger}M\boldsymbol{A} = (\boldsymbol{A}^{\dagger}T)(T^\dagger MT) (T^\dagger \boldsymbol{A}) = \boldsymbol{B}^{\dagger}D\boldsymbol{B}$, where $D$ is diagonal, containing the eigenvalues of $M$ on its diagonal, and we have defined new operators $\boldsymbol{B}^{\dagger}$ and $\boldsymbol{B}$.

% The reason a unitary transformation is not sufficient is that no such $T$ exists in general. For the new operators $\boldsymbol{B}^{\dagger}$ and $\boldsymbol{B}$ to satisfy the commutation relation $\boldsymbol{B}\otimes \boldsymbol{B}^{\dagger} -((\boldsymbol{B}^{\dagger})^T\otimes(\boldsymbol{B})^T)^T=J$ we get the requirement $T^{-1} = JT^\dagger J$ by theorem \ref{thm:non-unitary}. Theorem \ref{thm:Tform} showed that $T$ takes the form \eqref{eq:Tform},
% % \begin{gather*}
% %     T = 
% %     \begin{pmatrix}
% %     T_1 & T_2 \\
% %     T_2^* & T_1^* \\
% %     \end{pmatrix},
% % \end{gather*}
% meaning that $T_2$ has to be zero for $J T^\dagger J = T^\dagger$. We can therefore not assume that $T^\dagger = T^{-1}$ in general. Also Tsallis states that $T_2 = 0 \iff M_2=0$ \cite{Tsallis}, which explains why a unitary transformation was sufficient when considering the non-interacting SOC Bose gas, and why it would fail in the case of the weakly interacting Bose gas.  

\section{Negative Eigenvalues in Diagonal Hamiltonian}
Let us look at the example of BV diagonalizing a Hamiltonian $H = \boldsymbol{A}^{\dagger}M\boldsymbol{A}$, where $\boldsymbol{A} = (A_1, A_2, A_1^\dagger, A_2^\dagger)^T$ and $M$ is 
\begin{equation}
    M = 
    \begin{pmatrix}
    1 & -2 & 1 & 0 \\
    -2 & 1 & 0 & 0 \\
    1 & 0 & 1 & -2 \\
    0 & 0 & -2 & 1 \\
    \end{pmatrix}.
\end{equation}
The eigenvalues of $MJ$ are $\lambda_1 = 2\sqrt{2}$, $\lambda_2 = 1$, $\lambda_3 = -1$ and $\lambda_4 = -2\sqrt{2}$. Let $\boldsymbol{x}_i = (x_1, x_2, x_3, x_4)^T$ be general vectors. The equation for the first eigenvector is $MJ\boldsymbol{x}_1 = \lambda_1\boldsymbol{x}_1$. %It reads
% \begin{align}
%     \begin{split}
%         x_1-2x_2-x_3 &= 2\sqrt{2}x_1, \\
%         -2x_1+x_2 &= 2\sqrt{2}x_2, \\
%         x_1-x_3+2x_4 &= 2\sqrt{2}x_3, \\
%         2x_3 -x_4 &= 2\sqrt{2}x_4,
%     \end{split}
% \end{align}
% which becomes 
This set of equations reduces to
\begin{equation}
    x_1 = \frac{5+4\sqrt{2}}{2}x_4, \mbox{\qquad} x_2 = (-3-2\sqrt{2})x_4, \mbox{\qquad} x_3 = \frac{1+2\sqrt{2}}{2}x_4.
\end{equation}
It is obvious from this that $\boldsymbol{x}_1^\dagger J \boldsymbol{x}_1 > 0$ for any $x_4$. A BV normalized eigenvector can be chosen as
\begin{equation}
    \boldsymbol{x}_1 = \frac{1}{\sqrt{28+21\sqrt{2}}}\left(\frac{5+4\sqrt{2}}{2}, -3-2\sqrt{2}, \frac{1+2\sqrt{2}}{2}, 1\right)^T,
\end{equation}
and to be clear its BV norm is $\boldsymbol{x}_1^\dagger J \boldsymbol{x}_1 = 1$. We now know that $K\boldsymbol{x}_1$ will be an eigenvector corresponding to the eigenvalue $\lambda_4 = -\lambda_1 = -2\sqrt{2}$, and its BV norm is, by the definition of the operator $K$, given by $(K\boldsymbol{x}_1)^\dagger J (K\boldsymbol{x}_1) = -1$. 

%In fact, if we set $x_4 = a$ the norm is $\abs{a}^2(28+21\sqrt{2})$. 
%In fact, if we set $x_4 = a$ the norm is $\abs{a}^2(-7/4)$.

Turning to the eigenvalue $\lambda_2 = 1$, its corresponding eigenvector obeys $MJ\boldsymbol{x}_2 = \lambda_2\boldsymbol{x}_2$. %This set of equations reads
% \begin{align}
%     \begin{split}
%         x_1-2x_2-x_3 &= x_1, \\
%         -2x_1+x_2 &= x_2, \\
%         x_1-x_3+2x_4 &= x_3, \\
%         2x_3 -x_4 &= x_4,
%     \end{split}
% \end{align}
% which becomes 
This set of equations reduces to
\begin{equation}
    x_1 = 0, \mbox{\qquad} x_2 = -\frac{1}{2}x_4, \mbox{\qquad} x_3 = x_4.
\end{equation}
From this, it is clear that $\boldsymbol{x}_2^\dagger J \boldsymbol{x}_2 < 0$ no matter how we choose $x_4$. A BV normalized eigenvector can be chosen as
\begin{equation}
    \boldsymbol{x}_2 = \frac{2}{\sqrt{7}}\left(0, -\frac{1}{2}, 1, 1\right)^T,
\end{equation}
whose BV norm is $\boldsymbol{x}_2^\dagger J \boldsymbol{x}_2 = -1$. As above $K\boldsymbol{x}_2$ will be an eigenvector corresponding to $\lambda_3 = -\lambda_2 = -1$, but now it is this vector that has BV norm 1, $(K\boldsymbol{x}_2)^\dagger J (K\boldsymbol{x}_2) = 1$. We are forced to put the eigenvectors with positive BV norm in the left half of $T$ in order for the new operators $\boldsymbol{B} = T^\dagger \boldsymbol{A}$ to be bosonic. The requirement for this is $JT^\dagger JT = I$. If we construct $T$ as $T = [\boldsymbol{x}_1 | K\boldsymbol{x}_2 | K\boldsymbol{x}_1 | \boldsymbol{x}_2]$ we indeed find $JT^\dagger JT = I$. Additionally, we find that $T^{-1}MJTJ = D = \textrm{diag}(2\sqrt{2}, -1, 2\sqrt{2}, -1)$. In conclusion, the diagonalized Hamiltonian is
\begin{equation}
    H = \boldsymbol{B}^{\dagger}D\boldsymbol{B} = 2\sqrt{2}(2B_1^\dagger B_1+1) -1(2B_2^\dagger B_2 +1). 
\end{equation}

If on the other hand we try to insist on positive eigenvalues in the diagonal matrix, we can try to set up $T$ as $T = [\boldsymbol{x}_1 | \boldsymbol{x}_2 | K\boldsymbol{x}_1 | K\boldsymbol{x}_2]$. With this choice we do find $T^{-1}MJTJ = D = \textrm{diag}(2\sqrt{2}, 1, 2\sqrt{2}, 1)$, however,  $JT^\dagger JT = \textrm{diag}(1, -1, 1, -1) \neq I$, showing that $JT^\dagger J \neq T^{-1}$. Thus, defining $T$ in this alternative way means that the new operators are not bosonic.

\section{Alternate Approaches}
As mentioned, some authors use $JM$ instead of $MJ$ in their diagonalization procedure. We have shown that there is a clear relationship between both the eigenvalues and eigenvectors of these two matrices. They have the same eigenvalues, and if $\boldsymbol{x}$ is an eigenvector of $MJ$, then $J\boldsymbol{x}$ is an eigenvector of $JM$. The purpose of this section is to see if such proofs can be made for other alternate approaches as well, showing that the eigenvalues will not depend on the method we have chosen to obtain them. 

Considering once more the two approaches of diagonalizing $JM$ or $MJ$, it can even be shown that the definitions of the new operators are the same. In our approach, $\boldsymbol{B} = T^\dagger \boldsymbol{A}$. Meanwhile, in \cite{Xiao} $\boldsymbol{B} = T_X^{-1}\boldsymbol{A}$, where $T_X$ is such that $T_X^{-1} JM T_X$ is diagonal and $T_X^{-1} = JT_X^\dagger J$. From the form of $T$ and $T_X$ in the BV transformation, and the knowledge that if $\boldsymbol{x}$ is an eigenvector of $MJ$, then $J\boldsymbol{x}$ is an eigenvector of $JM$, we conclude that $T_X = JTJ$. Thus, $T_X^{-1} = JT_X^\dagger J = JJT^\dagger JJ = T^\dagger$, and therefore the two approaches define the new operators in the same way.

%-----------------------Bogoliubov, symplectic-------------------------------
% The usual Bogoliubov transformation employed to solve the weakly interacting Bose gas can be thought of as a symplectic transformation. In this case one can simplify the Hamiltonian such that a basis of length 2 is sufficient. The Bogoliubov transformation reads $\boldsymbol{B} = S^T\boldsymbol{A}$, or %opposite, and let u,v real
% \begin{gather}
%     \begin{pmatrix} B_{\boldsymbol{k}} \\   B_{-\boldsymbol{k}}^\dagger  \end{pmatrix} = \begin{pmatrix} u_{\boldsymbol{k}}^* & v_{\boldsymbol{k}} \\ v_{\boldsymbol{k}}^* & u_{\boldsymbol{k}}  \end{pmatrix} \begin{pmatrix} A_{\boldsymbol{k}} \\   A_{-\boldsymbol{k}}^\dagger  \end{pmatrix},
% \end{gather}
% where $|u_{\boldsymbol{k}}|^2-|v_{\boldsymbol{k}}|^2 = 1$ ensures the new operators are bosonic. The transformation matrix $S$ is such that $S^T \Omega S = \Omega$, where $\Omega$ is the matrix
% \begin{equation}
%     \Omega = \begin{pmatrix} 0 & I \\ -I & 0 \end{pmatrix}.
% \end{equation}
% The inverse of this matrix is its transpose, i.e. $\Omega^T \Omega = I$. The fact that the transformation matrix obeys $S^T \Omega S = \Omega$ is what makes this a symplectic transformation. We however note that $S^\dagger J S = J$ as well, so this is also a special case of a BV transformation. Setting up the transformation matrix $T$ in the BV transformation will in general be more straight forward than setting up the symplectic transformation matrix. It can be shown that the two approaches would yield the same eigenvalues, and the BV transformation will be preferred.


% Let us explore why we use a BV transformation in the general case instead of a symplectic transformation.

% Imagine we still have $\boldsymbol{A} = (A_1, \dots A_n, A_1^\dagger, \dots A_n^\dagger)^T$. To get the matrix $\Omega$ involved in our diagonalization, we need it to appear in the commutation relations of the operator vectors. The way to do this is to replace $\boldsymbol{A}^\dagger$ by $\boldsymbol{A}^T = (A_1, \dots A_n, A_1^\dagger, \dots A_n^\dagger)$. Then we have $\boldsymbol{A}\otimes \boldsymbol{A}^{T} -(\boldsymbol{A}\otimes \boldsymbol{A}^T)^T=\Omega$. We define the new operators by $\boldsymbol{B}^T = \boldsymbol{A}^T S$ and hence we must have $\boldsymbol{B} = S^T \boldsymbol{A}$. For these to satisfy the same commutation relation $\boldsymbol{B}\otimes \boldsymbol{B}^{T} -(\boldsymbol{B}\otimes\boldsymbol{B}^T)^T=\Omega$ we get the requirement $S^T \Omega S = \Omega$, i.e. a symplectic transformation. Alternatively the requirement of bosonic pseudoparticles can be written $S^T = \Omega S^{-1} \Omega^T$. We can connect the new matrix $M_s$ here to the old matrix $M$ in the BV approach by $M_s = \Sigma_x M$ because replacing $\boldsymbol{A}^\dagger$ by $\boldsymbol{A}^T$ is the same as moving the last $n$ rows of $M$ above the first $n$ rows. We can define the diagonalization as
% \begin{align}
%     \begin{split}
%         &\boldsymbol{A}^T M_s \boldsymbol{A} = \boldsymbol{A}^T (SS^{-1})M_s (\Omega(S(\Omega^T \Omega)S^{-1})\Omega^T)\boldsymbol{A} \\
%         &=  (\boldsymbol{A}^T S)(S^{-1}M_s\Omega S)\Omega^T (\Omega S^{-1} \Omega^T\boldsymbol{A}) = \boldsymbol{B}^T R\Omega \Omega^T \boldsymbol{B} = \boldsymbol{B}^T R \boldsymbol{B}.
%     \end{split}
% \end{align}
% Thus, it is $M_s\Omega$ we are diagonalizing and its eigenvalues will enter the diagonal matrix $R\Omega$. The matrix $R$ is not diagonal, but is has the exact form needed for $H$ to end up in diagonal form. Assume $\boldsymbol{x}$ is an eigenvector corresponding to the eigenvalue $\lambda$ of $MJ$. Using that
% \begin{equation}
%     \Omega^T J = \begin{pmatrix} 0 & -I \\ I & 0 \end{pmatrix} \begin{pmatrix} I & 0 \\ 0& -I \end{pmatrix} = \begin{pmatrix}0&I\\I&0\end{pmatrix} = \Sigma_x,
% \end{equation}
% we find
% \begin{equation}
%     MJ\boldsymbol{x} = \lambda \boldsymbol{x} \iff \Sigma_x M (\Omega \Omega^T) J \boldsymbol{x} = \lambda \Sigma_x \boldsymbol{x} \iff M_s\Omega (\Sigma_x \boldsymbol{x}) = \lambda (\Sigma_x \boldsymbol{x}).
% \end{equation}
% This proves that $MJ$ and $M_s \Omega$ have the same set of eigenvalues, and that if $\boldsymbol{x}$ is an eigenvector of $MJ$, then $\Sigma_x\boldsymbol{x}$ is an eigenvector of $M_s \Omega$. It appears setting up the matrix $S$ that performs this symplectic transformation will be more challenging than setting up the matrix $T$ that performs the BV transformation. As the eigenvalues are the same, the two approaches should lead to the same diagonalized Hamiltonian, and the BV transformation will be preferred.

Next, we consider what happens if we change the basis by interchanging some entries in $\boldsymbol{A}$ and thus simultaneously in $\boldsymbol{A}^\dagger$. This will result in the simultaneous interchange of two rows and two columns in $M$. Such interchanges can be represented by matrices $P^{ij}$, where $P^{ij}$ is the result of interchanging row $i$ and $j$ in $I$. We note that $P^{ij} = P^{ji}$ and that $(P^{ij})^2 = I$. 
% An example when $n=2$ is
% \begin{equation}
%     P^{23}=\begin{pmatrix}
%     1 & 0 & 0 & 0\\
%     0 & 0 & 1 & 0 \\
%     0 & 1 & 0 & 0 \\
%     0 & 0 & 0 & 1
%     \end{pmatrix}.
% \end{equation}

The new matrix after interchanging elements $i$ and $j$ of $\boldsymbol{A}$ and $\boldsymbol{A}^\dagger$ is $P^{ij}MP^{ij}$. When changing the basis we are also altering the commutation relation. The new result of the commutation relation is in fact $P^{ij}JP^{ij}$, which will replace $J$ in the diagonalization procedure. Hence, it is $P^{ij}MP^{ij}P^{ij}JP^{ij} = P^{ij}MJP^{ij}$ we are diagonalizing. Our starting point is the eigenvalue relation $MJ\boldsymbol{x} = \lambda \boldsymbol{x}$. By matrix manipulations we obtain
\begin{align}
    \begin{split}
        MJ\boldsymbol{x} = \lambda \boldsymbol{x} &\iff P^{ij}MJ(P^{ij}P^{ij})\boldsymbol{x} = \lambda P^{ij}\boldsymbol{x} \\
        &\iff (P^{ij}MJP^{ij})(P^{ij}\boldsymbol{x}) = \lambda (P^{ij}\boldsymbol{x}).
    \end{split}
\end{align}
This shows that $MJ$ and $P^{ij}MJP^{ij}$ have the same eigenvalues and that if $\boldsymbol{x}$ is an eigenvector of $MJ$, then $P^{ij}\boldsymbol{x}$ in an eigenvector of $P^{ij}MJP^{ij}$.

Finally, one may ask what happens if one preemptively transforms $M$ before attempting to diagonalize. The question is whether $S^{-1} M S J$ and $MJ$ have the same eigenvalues, assuming the temporary new operators are bosonic, and obey the same commutation relations as the original operators. 
\begin{align}
    \begin{split}
    MJ\boldsymbol{x} = \lambda \boldsymbol{x} &\iff S^{-1} M(S(JJ)S^{-1})J\boldsymbol{x} = \lambda S^{-1}\boldsymbol{x} \\
    &\iff  S^{-1} MSJ(JS^{-1}J\boldsymbol{x}) = \lambda (S^{-1}\boldsymbol{x}).
    \end{split}
\end{align}
The eigenvalues are the same only if $JS^{-1}J = S^{-1}$. If $S$ has the form
\begin{gather*}
    S = \begin{pmatrix}
    S_1 & S_2 \\
    S_3 & S_4
    \end{pmatrix},
\end{gather*}
this is true if $S_2 = S_3 = 0$. An example where $JS^{-1}J = S^{-1}$, is if we transform the Hamiltonian we are considering for a SOC, weakly interacting BEC to the helicity basis \eqref{eq:Helicitybasis} before attempting to diagonalize. Hence, such a transformation will in general not be interesting as it will yield the same eigenvalues. More generally, we can say that $JS^{-1}J = S^{-1}$ will be true for any transformation $C_i = c_{i1} A_1 + \dots+ c_{in} A_n$, i.e. one where the Hermitian conjugate of any $A_j$ does not enter the definition of the temporary new operators $C_i$.
